Regret Bounds for Generalized Linear Bandits under Parameter Drift

Generalized Linear Bandits (GLBs) are powerful extensions to the Linear Bandit (LB) setting, broadening the benefits of reward parametrization beyond linearity. In this paper we study GLBs in non-stationary environments, characterized by a general metric of non-stationarity known as the variation-budget or \emph{parameter-drift}, denoted $B_T$. While previous attempts have been made to extend LB algorithms to this setting, they overlook a salient feature of GLBs which flaws their results. In this work, we introduce a new algorithm that addresses this difficulty. We prove that under a geometric assumption on the action set, our approach enjoys a $\tilde{\mathcal{O}}(B_T^{1/3}T^{2/3})$ regret bound. In the general case, we show that it suffers at most a $\tilde{\mathcal{O}}(B_T^{1/5}T^{4/5})$ regret. At the core of our contribution is a generalization of the projection step introduced in Filippi et al. (2010), adapted to the non-stationary nature of the problem. Our analysis sheds light on central mechanisms inherited from the setting by explicitly splitting the treatment of the learning and tracking aspects of the problem.

==> challenges.tex <==
\newpage
\section{Challenges and main contribution {\color{red}(old)}}
\label{sec:challenges}

\paragraph{On the crucial role of $\pmb{\Rm}$.}
A fundamental difference between the \lb{} and \glb{s} arise from the fundamentally different \emph{learning} difficulties that take place in both settings. The magnitude of this difference is embodied by the ratio $R_\mu\defeq\km/\cm$, which can be understood as a measure of the non-linearity of the inverse link function . Indeed in the linear case $R_\mu=1$, while easy computations show that for the logistic bandit and Poisson bandit $R_\mu\geq e^{XS}$ (up to multiplicative constants), hence $R_\mu$ grows exponentially large with the diameter of the decision set. From a technical point of view, this problem-dependent constant allows to link the \emph{prediction error} of an admissible parameter to its \emph{trajectory deviation}, which is key step in the design of exploration bonuses. Formally:
	\begin{align}
		\forall (x,\theta)\in\mcal{X}\times\Theta\quad \mu(\langle x,\theta\rangle)- \mu(\langle x,\ts{t} \rangle) \leq R_\mu \lVert x\rVert_{\mbold{V_t^{-1}}} \lVert\underbrace{ g_t(\theta)-g_t(\ts{t})}_{\text{trajectory deviation}}\rVert_{\mbold{V_t^{-1}}}
		\label{eq:rmu_characterization}
	\end{align}
	 Previous attempts in the non-stationary setting \citep{cheung2019learning, zhao2020simple} uses this tool (along with some concentration results) to characterize the \emph{prediction error} of $\hat{\theta}_t$. Unfortunaly, this approach is mistaken. Indeed, it is important to realize that the characterization \eqref{eq:rmu_characterization} holds \textbf{only} over the decision set, however it was never proven that $\lVert \hat{\theta}_t \rVert_2\leq S$. Unfortunately, this is not easily fixed, on the contrary. Indeed, existing tail-inequalities from the \lb{} literature rather suggest that in some directions, $\hat\theta_t$ is can be distant from the $\ts{t}$ by a factor growing as $\log(t)$. Given the exponential growth of $R_\mu$ with the diameter of the decision set, inflating it enough to contain $\hat{\theta}_t$ will lead to a dramatic loss in performance. A correct analysis requires additional work to map the parameters of interest back to \emph{admisssible} parameters in the decision set.
		
	\paragraph{Feasible projections.} In the stationary setting, \cite{filippi2010parametric} achieve this by \emph{projecting} (according to an appropriate metric) $\hat{\theta}_t$ back to the decision set. This strategy is also employed by \cite{russac2020algorithms} in the abrupt-changing environment. Formally, they compute:
	\begin{align*}
		\tilde{\theta}_t \defeq \argmin_{\ltwo\theta\leq S} \lVert g_t(\theta)-g_t(\hat{\theta}_t)\rVert_{\mathbf{\widetilde{V}_t^{-1}}}
	\end{align*}
	to be used to predict rewards. Since $\tilde{\theta}_t$ is admissible, Equation~\eqref{eq:rmu_characterization}  applies. Further, thanks to the contracting nature of the projection, one can relate the trajectory deviations of $\tilde{\theta}_t$ and $\hat{\theta}_t$, respectively. In an abruptly changing environment, this is enough to conclude the analysis as the latter can be controlled thanks to existing concentration inequalities Intuitively, \emph{far from a switch}, $\hat{\theta}_t$ concentrates around $\ts{t}$ and the problem boils down to a stationary study. The situation is quite different is a slowly-varying environment, as $\hat{\theta}_t$ does not "concentrate" around $\ts{t}$, but around a \emph{tracking parameter} $\bar{\theta}_t$. This parameter is at the heart of our analysis, as it naturally separates two key mechanisms in non-stationary bandits: \emph{learning} ($\hat{\theta}_t\to\bar\theta_{t}$) and \emph{tracking} ($\bar\theta_{t}\to\ts{t})$. For technical reasons we omit for now in the sake of conciseness, \textcolor{red}{these two processes evolve at different rates}, and therefore need to be controlled thanks to different metrics. This matter therefore calls for an innovative mechanism to map $\hat{\theta}_t$ back to an admissible parameter. 

\input{tikz_figure}

\paragraph{A solution sketch.} We will give here the main intuition behind our proposed solution. We introduce: 
\begin{align*}
	\mathcal{E}_t^{\delta}(\theta) = \left( \theta' \text{ s.t } \lVert g_t(\theta') - g_t(\theta) \rVert_{\mathbf{\widetilde V_t^{-1}}} \leq \beta_\delta \right).
\end{align*}
Anticipating some later results, we will construct $\beta_\delta$ such that $\bar\theta_t\in\mcal{E}_\delta(\hat{\theta}_t)$ with high probability. Unlike in the stationary case (where $\bar\theta_t=\ts{1}$), this last confidence set might not intersect the set of admissible parameters (another reason a "projection" does not work). However, we will show that the drift of $\mcal{E}_t^\delta(\hat{\theta}_t)$ is linked to the variation budget $B_T$. A valid strategy is therefore to look for the optimal (w.r.t a particular metric) \emph{vibration} of the confidence sets $\mcal{E}_t^\delta(\hat{\theta}_t)$, such that it intersect the admissible set. This intuition can be formalized through the following program: 
\begin{align}
	\theta_t^p \in \argmin_\theta \left\{\lVert g_t(\theta) - g_t(\hat\theta_t) \rVert_{\mathbf{\widetilde V_t^{-2}}}\right\} \text{ s.t } \Theta \cap \mathcal{E}_t^\delta(\theta) \neq \emptyset
	\tag{OPT1}
\end{align}
Note that any parameter $\tilde{\theta}_t\in\mcal{E}_t^\delta(\theta_t^p)$ is admissible, and we will show that the different parameters obey the following scaling:
\begin{align*}
	bla
\end{align*}
which will allow us to derive a valid regret bound.







==> tikz_figure.tex <==
\begin{figure}
\centering
\scalebox{1.2}{
    \begin{tikzpicture}
     \begin{axis}[
     	axis equal,
        axis x line=none,
        axis y line=none,
        xtick=\empty,
        ytick=\empty,
        scaled ticks=false,
        xmin=-20,
        xmax=20,
        ymin=-20,
        ymax=20,
        xlabel=,
        ylabel=,
   ]
   \def\radiusT{8}
   
   \fill[pattern=north west lines, pattern color=blue, opacity=0.5] 
  (axis cs:0,0) circle [radius=\radiusT];
  \draw[color=blue, line width=1.5] (axis cs:0,0) circle [radius=\radiusT];
   \node at (axis cs:-\radiusT,-\radiusT) {$\color{blue}\Theta$};
   
   \fill[color=black, line width=1.2, pattern= horizontal lines, opacity=0.2] plot [smooth cycle, tension=1] coordinates {(axis cs: 7,13) (axis cs: 18,9) (axis cs: 17,13) (axis cs: 7,16)} node at (axis cs:9,14) {};
   \draw[color=black, line width=1.2] plot [smooth cycle, tension=1] coordinates {(axis cs: 7,13) (axis cs: 18,9) (axis cs: 17,13) (axis cs: 7,16)} node at (axis cs:9,14) {};
   
     \draw[color=black, line width=1.2, draw opacity=0.4] plot [smooth cycle, tension=1] coordinates {(axis cs: 4.5,7) (axis cs: 15.5,3) (axis cs: 14.5,7) (axis cs: 4.5,10)} node at (axis cs:9,14) {};
   
   % theta_hat
   \node at (axis cs:12.5,13) {\scriptsize$\hat{\theta}_t$};
   \draw[fill=black, color=black] (axis cs: 11,13) circle [radius=0.3];
   \node at (axis cs:15,17) {\scriptsize$\mathcal{E}_t^{\delta}(\hat{\theta}_t)$};
   % theta_bar
     \node at (axis cs:17.5,11) {\scriptsize$\bar{\theta}_t$};
     \draw[fill=black, color=black] (axis cs: 16,11) circle [radius=0.3];
   % theta_star
   \node[align=right] at (axis cs:7.75+3,2) {\scriptsize$\theta_{t}^{\star}$};
   \draw[fill=black, line width=1.5] (axis cs:7.75,2) circle [radius=0.3];
   % theta_p
   \node[align=right] at (axis cs:10,7) {\scriptsize $\theta_t^{p}$};
   \draw[fill=black, color=black, draw opacity=0.5] (axis cs: 8.5,7) circle [radius=0.3];
   % theta_tilde
   \draw[fill=red, color=red, draw opacity=0.5] (axis cs: 4., 7) circle [radius=0.3];
   \node[color=red] at (axis cs: 5.2,8.2) {\color{red}\scriptsize$\tilde{\theta}_t$};

   % scale between theta_p and theta_bar 
   \draw[<->] (axis cs:21,7) -- (axis cs: 12.75,-2);
   \draw[dotted] (axis cs: 7.75,2) -- (axis cs: 12.75,-2);
   \draw[dotted] (axis cs: 16,11) -- (axis cs: 21,7);
   \node[align=right, rotate=53] at (axis cs: 18.5,1.5) {\footnotesize$\sim\! B_t$};
   
   % scale between theta_pt and theta_hat
   \draw[dotted] (axis cs: 2, 16.75) -- (axis cs:11,13);
   \draw[dotted] (axis cs: -0.5, 10.75) -- (axis cs:8.5,7);
   \draw[<->] (axis cs: 2, 16.75) -- (axis cs: -0.5, 10.75);
   \node[align=right, rotate=70] at (axis cs: -1, 14.5) {\footnotesize$\sim \! B_t$};
    \end{axis}
    \end{tikzpicture}}
    \vspace{-40pt}
    \caption{Illustration of the different parameters of interest. As stated by Lemma~\ref{lemma:bound_first_drift} and Lemma~\ref{lemma:bound_second_drift}, the deviations ($\theta_t^p\leftrightarrow \hat\theta_t$) and ($\bar\theta_t\leftrightarrow\ts{t}$) are linked to the parameter-drift $B_t$. On the other hand, the deviations  ($\hat\theta_t\leftrightarrow \bar\theta_t$) and  ($\tilde\theta_t\leftrightarrow \theta_p^t$) are characterized by the stochastic nature of the problem.}
    \label{fig:lemmaseconddriftillustration}
\end{figure}
